Collaborative Object Transportation Using MAVs via Passive Force Control

This paper shows a strategy based on passive force control for collaborative object transportation using Micro Aerial Vehicles (MAVs), focusing on the transportation of a bulky object by two hexacopters. The goal is to develop a robust approach which does not rely on: (a) communication links between the MAVs, (b) the knowledge of the payload shape and (c) the position of grasping point. The proposed approach is based on the master-slave paradigm, in which the slave agent guarantees compliance to the external force applied by the master to the payload via an admittance controller. The external force acting on the slave is estimated using a non-linear estimator based on the Unscented Kalman Filter (UKF) from the information provided by a visual inertial navigation system. Experimental results demonstrate the performance of the force estimator and show the collaborative transportation of a 1.2 m long object.

==> sections/implementation.tex <==
\section{FORCE AND TORQUE ESTIMATOR}
In this section we derive a discrete time model for the rotational and translational dynamic of an hexacopter and describe the UKF based force and torque estimator.
\subsection{Hexacopter Model with External Force and Torque}
In this section we derive a nonlinear, discrete time model for the rotational and translational dynamic of an hexacopter, to be used in the prediction step of the force and torque estimator. 
\paragraph{Model Assumptions}
In order to simplify the model derivation, we assume that: 
\begin{itemize}
	\item The MAV structure is rigid, symmetric on the ${x_{B}y_{B}}$ and $y_{B}z_{B}$ planes, and the CoG and body frame origin \textit{B} coincide;
	\item Aerodynamic interaction with the ground or other surfaces can be neglected and we can consider only dominant aerodynamic effects at low speed;
	\item No external torque acts around $x_B$ and $y_B$ axis.
\end{itemize}

\par
In addition, we define the rotation matrix from frame $B$ to frame $I$ as 
$\boldsymbol{R(q)}_{B}^{I}$, where $\boldsymbol{q}$ is the normalized quaternion representing the attitude of the vehicle. Last, we simplify the equations by introducing $U_{1}$, $U_{2}$ and $U_{3}$ as the total torque produced by the propellers around, respectively, $x_b$, $y_b$ and $z_b$, and $U_{4}$ as the total thrust produced by the propellers expressed in $B$ frame. We compute $U_{i}, i = 1\dots4$ from the rotor speed $n_{i}$, $i=1\dots6$, using the allocation matrix, as defined in \cite{Achtelik2013} for the AscTec Firefly hexacopter \cite{asctec}:

 \begin{equation}
 \begin{bmatrix}
 U_{1} \\ U_{2} \\ U_{3} \\ U_{4} \\
 \end{bmatrix}
 =
 \mathbf{K}
 \begin{bmatrix}
  s & 1 & s & -s & -1 & s \\
-c & 0 & c & c & 0 & -c \\
-1 & 1 & -1 & 1 & -1 & 1 \\
 1 & 1 & 1 & 1 & 1 & 1
 \end{bmatrix}
 \begin{bmatrix}
 {n_{1}}^2 \\
 \vdots \\
 {n_{6}}^2\\
 \end{bmatrix}
 \end{equation}
 
 \begin{equation}
  \mathbf{K} = 
  \text{diag}
   \big(
    \begin{bmatrix}
    l k_n& l k_n& k_n k_m& k_n
    \end{bmatrix}
   )
 \end{equation} 
where $l$ is the boom length, $k_n$ and $k_m$ are rotor constants and $c = \text{cos}(30\deg)$ and $s = \text{sin}(30\deg)$.
 
\paragraph{Translational Dynamics}
We derive the linear acceleration with respect to $I$ reference frame by taking into account the following forces: (a) gravity, (b) thrust, (c) aerodynamic effects, (d) external forces due to interaction with the vehicle. We obtain:
\begin{equation}
	\begin{bmatrix}
		\ddot{x} \\
		\ddot{y} \\
		\ddot{z}
	\end{bmatrix} 
	= \frac{1}{m}\boldsymbol{R(q)}_{B}^{I} \Bigg(
	\begin{bmatrix}
	0\\
	0\\
	U_{4}\\
	\end{bmatrix}
	+\boldsymbol{ F}^{aero}
	\Bigg) 
	-
	\begin{bmatrix}
	0\\0\\g
	\end{bmatrix}
		+ 
	\frac{1}{m} \boldsymbol{F}^{ext}
	\label{transldyn}
\end{equation}
where $\boldsymbol{F}^{ext}$ are the external forces that act on the vehicle expressed in $I$ reference frame, $m$ is the mass of the vehicle, and $\boldsymbol{F}^{aero}$ is defined according to \cite{RDlecture} as: 
\begin{equation}
\boldsymbol{F}^{aero} = k_{drag} \sum_{i=1}^{6}|n_{i}|
\begin{bmatrix}
\dot{x} \\
\dot{y} \\
0
\end{bmatrix}
\end{equation}

\paragraph{Rotational Dynamics}
We derive the angular acceleration $\dot{\boldsymbol{\omega}}$ in $B$ frame by taking into account the following torques: (a) total torque produced by propellers, (b) external torque around z axis, (c) inertial effects, (d) propeller's gyroscopic effects. We obtain:
\begin{equation}
\boldsymbol{\dot{\omega}} = \mathbf{J}^{-1}
\Bigg(
\begin{bmatrix} 
U_{1} \\
U_{2} \\
U_{3} \\
\end{bmatrix}
+
\begin{bmatrix}
0\\
0\\
\tau^{ext}
\end{bmatrix}
- \boldsymbol{\omega }\times \mathbf{J}\boldsymbol{\omega} 
- \boldsymbol{\tau^{rotor}}
\Bigg) \label{rotdyn}
\end{equation}
where $\tau_{ext}$ is the external torque around the $z_B$ axis.
$ \mathbf{J}$ is the inertia tensor of the MAV with respect to  $B$  frame, defined as
\begin{equation}
\mathbf{J} = 
\begin{bmatrix}
J_{xx} & 0 & 0 \\
0 & J_{yy} & 0 \\
0 & 0 & J_{zz} 
\end{bmatrix}
\end{equation}
and $\tau_{rotor}$ is the torque caused by propeller's gyroscopic effects defined according to \cite{Bouabdallah2007} as
\begin{equation}
\boldsymbol{\tau_{rotor}} = J_{r}\Omega_{r}
\begin{bmatrix}
\omega_{y}\\
\omega_{x}\\
0
\end{bmatrix}
\textrm{with } 
\Omega_{r}  = \sum_{i = 1}^{6} n_{i} - 6 \omega_z
\end{equation}
where $J_r$ is the propeller's moment of inertia around its axis of rotation.

%%% DISCRETIZATION %%% 
\paragraph{Discretized Model}
The analytic models (\ref{transldyn})  and (\ref{rotdyn}) have been discretized using the forward Euler method, given the sampling time $T_s = 0.01$s. 

\par
First, for the rotational dynamics, we rewrite (\ref{rotdyn}) as 
\begin{equation}
\boldsymbol{\dot{\omega}} = f_{rot}(\boldsymbol{\omega}_k, \boldsymbol{n}_k, \tau_k^{ext}) 
\end{equation} 

with $\omega_k = \omega(T_s k)$ and $\boldsymbol{n}$ being the vector containing the speed of each propeller at the current time.

We obtain the discretized rotational dynamic
\begin{equation}
\label{d_ang_vel}
\boldsymbol{\omega}_{k+1} = 	\boldsymbol{\omega}_k + T_sf_{rot}(\boldsymbol{\omega}_k, \boldsymbol{n}_k, \tau_{k}^{ext})
\end{equation}

We define $\boldsymbol{q}_k$ as the normalized attitude quaternion at time-step $k$. The attitude quaternion is integrated using the method proposed in \cite{Cheon2007}
\begin{equation}
\label{d_att}
\boldsymbol{q}_{k+1} = \boldsymbol{\Omega}(\boldsymbol{\omega}_k) \boldsymbol{q}_k
\end{equation}
with 
\begin{equation}
\boldsymbol{\Omega}(\boldsymbol{\omega}_k) = 
\begin{bmatrix}
\cos(\frac{1}{2}\norm{\boldsymbol{\omega}_k} T_s) \mathbf{I}_{3 \times 3}  & \mathbf{\Psi}_k \\
-\mathbf{\Psi}_k^T &  \cos(\frac{1}{2}\norm{\boldsymbol{\omega}_k} T_s)  
\end{bmatrix} 
\end{equation}
and 
\begin{equation}
\mathbf{\Psi}_k = \sin{(\frac{1}{2} \norm{\boldsymbol{\omega_k}}T_s)}\boldsymbol{\omega_k}/\norm{\boldsymbol{\omega_k}}
\end{equation}

Second, for the translational dynamics we rewrite (\ref{transldyn}) as 
\begin{equation}
\dot{\boldsymbol{v}}= f_{transl}(\boldsymbol{q}_k, \boldsymbol{\omega}_k, \boldsymbol{n}_k, \boldsymbol{F}_k^{ext})
\end{equation}
with $\boldsymbol{v} = [\dot{x}, \dot{y}, \dot{x}]^T$.  In addition we define $\boldsymbol{p} = [x, y, z]^T$ and we derive the discretized translational dynamic equation 
\begin{equation}
\label{d_vel}
\boldsymbol{v}_{k+1} = \boldsymbol{v}_k + T_s f_{transl}(\boldsymbol{q}_k, \boldsymbol{\omega}_k, \boldsymbol{n}_k, \boldsymbol{F}_k^{ext})
\end{equation}
\begin{equation}
\label{d_pos}
\boldsymbol{p}_{k+1}= \boldsymbol{p}_k+ \boldsymbol{v}_k T_s + 	\frac{1}{2} T_s^2 f_{transl}(\boldsymbol{q}_k, \boldsymbol{\omega}_k, \boldsymbol{n}_k, \boldsymbol{F}_k^{ext})
\end{equation}
\par
Last, we rewrite (\ref{d_ang_vel}), (\ref{d_att}), (\ref{d_vel}) and (\ref{d_pos}) as 
\begin{equation}
\label{discr:dynold}
\boldsymbol{{s}}_{k+1}= f(\boldsymbol{{s}}_k, \boldsymbol{F}_k^{ext}, 	\tau_k^{ext}, \boldsymbol{n}_{k})
\end{equation}
with 
\begin{equation}
\label{discr:state}
\boldsymbol{{s}}_k =
\begin{bmatrix}
\boldsymbol{p}_k&\boldsymbol{v}_k & \boldsymbol{q}_k & \boldsymbol{\omega}_k
\end{bmatrix}
\end{equation}
From now on we will change the notation used in (\ref{discr:dynold}), where $\boldsymbol{n}_{k}$ is explicitly expressed; we introduce the notation
\begin{equation}\label{discr:dyn}
\boldsymbol{s}_{k+1} = f_k(\boldsymbol{s}_k, \boldsymbol{F}_k^{ext}, 	\tau_k^{ext})
\end{equation}
where the dependency of $f(\cdot)$ from $\boldsymbol{n}_{k}$ is taken into account by making $f(\cdot)$ time-variant.

%%% FORCE AND TORQUE ESTIMATOR %%% 
\subsection{Force and Torque Estimator}
In this section we present the Unscented Kalman Filter (UKF) derived to estimate the external force and torque acting on the MAV. 

\paragraph{Process and Measurement models}
First, we augment the state vector of the hexacopter model (\ref{discr:state}) and the system dynamic equation (\ref{discr:dyn}) so that they take into account  the external force and torque.
We obtain:
\begin{equation}
{\boldsymbol{s}}_{k+1} = {f}_k({\boldsymbol{s}}_k) + \bar{\boldsymbol{w}}_k
\end{equation}
\begin{equation} \label{ukf:pred:sysdyn}
\boldsymbol{s}_k = 
\begin{bmatrix}
\boldsymbol{p}_k&\boldsymbol{v}_k&\boldsymbol{q}_k&\boldsymbol{\omega}_k&\boldsymbol{F}_k^{ext}&\tau_k^{ext} 
\end{bmatrix}
\end{equation}
We assume that the change of external force and torque is purely driven by zero mean additive process noise, whose covariance is a tuning parameter of the filter. The external force and torque are updated according to 
\begin{equation}
\begin{aligned}
&\boldsymbol{F}_{k+1}^{ext} = \boldsymbol{F}_{k}^{ext} \\ 
& \tau_{k+1}^{ext} = \tau_{k}^{ext} \\
\end{aligned}  
\end{equation}
or by assuming first-order dynamics expressed by 
\begin{equation}
\begin{aligned}
&\boldsymbol{F}_{k+1}^{ext} = \boldsymbol{F}_{k}^{ext} + T_s \dot{\boldsymbol{F}}^{ext}\\ 
& \tau_{k+1}^{ext} = \tau_{k}^{ext} + T_s \dot{\boldsymbol{\tau}}^{ext}
\end{aligned}  
\end{equation}
where $\dot{\boldsymbol{F}}^{ext}$ and $\dot{\boldsymbol{\tau}}^{ext}$ are constants set by the user and define the convergence speed of the estimates. 
In order to define the state covariance and the process noise covariance, we introduce a new representation $\bar{\boldsymbol{s}}_{k}$ of the state ${\boldsymbol{s}}_{k}$, where we substitute the attitude quaternion $\boldsymbol{q}_k$ with a $3 \times 1$ attitude error vector $\boldsymbol{e}_k$. More details about this substitution are explained in \ref{ukf:attitude}.
\begin{equation}
\bar{\boldsymbol{s}}_k = 
\begin{bmatrix}
\boldsymbol{p}_k&\boldsymbol{v}_k&\boldsymbol{e}_k& \boldsymbol{\omega}_k& \boldsymbol{F}_k^{ext}& \tau_k^{ext} \\
\end{bmatrix}
\end{equation}
 We can now introduce $\boldsymbol{P}_k$, the $16 \times 16$ covariance matrix associated to the state $\bar{\boldsymbol{s}}_k$, and $\boldsymbol{Q}$, the $16 \times 16$ time invariant  process noise diagonal covariance matrix.

%The time invariant $16 \times 16 $ process noise diagonal covariance matrix is
%\begin{equation}
%\boldsymbol{Q} =  \text{diag}(
%\begin{bmatrix}
%\boldsymbol{1}_3^T \sigma_{p,p}^2& 
%\boldsymbol{1}_3^T \sigma_{p,v}^2&
%\boldsymbol{1}_3^T \sigma_{p,e}^2& 
%\boldsymbol{1}_3^T  \sigma_{p,\omega} ^2& 
%{\sigma_{p,F}^{xy}}^2& {\sigma_{p,F}^{xy}}^2& %{\sigma_{p,F}^{z}}^2& \sigma_{p,\tau}^2
%\end{bmatrix}
%)
%\end{equation}
%where $\sigma_{p,e}$ is the process uncertainty associated to the 3 states attitude error vector (see \ref{ukf:attitude}).


Last, we define the measurement vector $\boldsymbol{z}_k$, the  associated $12 \times 12$ measurement noise covariance matrix $\boldsymbol{R}$ and the linear measurement function 
$\boldsymbol{z}_k  = \boldsymbol{H}{\bar{\boldsymbol{s}}}_k + \boldsymbol{v}_k $, under the assumption that the measurements are subject to zero-mean additive noise.
\begin{equation}
\boldsymbol{z}_k = 
\begin{bmatrix}
\label{ukf:meas_vect}
\boldsymbol{p}_k^m& \boldsymbol{v}_k^m& \boldsymbol{e}_k^m& 	\boldsymbol{\omega}_k^m
\end{bmatrix}
\end{equation}

\begin{equation} \label{ukf:meas_funct}
\begin{aligned}
\boldsymbol{z}_k & = \boldsymbol{H}{\bar{\boldsymbol{s}}}_k + \boldsymbol{v}_k \\
\boldsymbol{H} =  &
\begin{bmatrix}	
\mathbf{I}_{12\times12} & \mathbf{0}_{12 \times 4}
\end{bmatrix}
\end{aligned}
\end{equation}
\begin{equation} \label{ukf:meas_cov}
\boldsymbol{R} = 
\text{diag}(
\begin{bmatrix}
\boldsymbol{1}_3^T \sigma_{m,p}^2& 
\boldsymbol{1}_3^T \sigma_{m,v}^2&
\boldsymbol{1}_3^T \sigma_{m,e}^2& 
\mathbf{1}_3^T  \sigma_{m,\omega} ^2
\end{bmatrix}
)
\end{equation}

As a remark, we observe that the measured attitude quaternion is converted in a three states parametrization $\boldsymbol{e}_k$ for the measurement vector. In addition, the measurement update step of the filter is performed using the state vector $\bar{\boldsymbol{s}}_k$. (\ref{ukf_simpl_updt}).

\paragraph{Notation Declaration}
From now on, we will use the following notation:
\begin{itemize}
	\item $\hat{\boldsymbol{s}}_{k-1}^{+}$ denotes the estimated state before the prediction step
	\item $\hat{\boldsymbol{s}}_{k}^{-}$ denotes the estimated state after the prediction step and before the update step
	\item $\hat{{\boldsymbol{s}}}_{k}^{+}$ denotes the estimated state after the update step 
\end{itemize}
The same applies for the state covariance matrix  $\boldsymbol{P}$.

\paragraph{Prediction Step for Position, Velocity, Angular Velocity, External Force and Torque}
The predicted state for all the states with the exception of the attitude is computed using the standard UKF prediction step, as explained in \cite{Simon2006} and \cite{Julier1996}. The matrix square root is computed using the Cholesy decomposition \cite{Simon2006}.

\paragraph{Quaternion Based Attitude Estimation}
\label{ukf:attitude}
Quaternions do not naturally fit the Unscented Transformation (UT) since they are defined on a non linear manifold, while the UT is performed on a vector space. Interpreting a quaternion as a member of $\mathbb{R}^4$ produces a singular $4 \times 4$ covariance matrix and does not  guarantee the unitary norm constraint, while considering quaternions as members of $\mathbb{R}^3$ - by exploiting the unitary norm constraint - always produces a singularity. For these reasons we estimate the MAV attitude by following the approach proposed by \cite{Crassidis2003}  and \cite{Kraft2003}. The estimation is based on the error attitude quaternion with a three states parametrization obtained through the Modified Rodriguez Parameters (MRP). 

\textbf{Modified Rodriguez Parameters}
Let $\boldsymbol{q} = [\boldsymbol{q}_v^T, {q}_s]$ be a quaternion, where $\mathbf{\boldsymbol{q}_v}$ is the vector part and $q_s$ is the scalar part. A corresponding (but singular) attitude representation $\mathbf{p}$, with $\mathbf{p} \in \mathbb{R}^3$, can be obtained as
\begin{equation} \label{mrp:fromquat}
\mathbf{p} = f \frac{\mathbf{\boldsymbol{q}_v}}{a+q_s} 
\end{equation}
where $a$ is a parameter from 0 to 1 and f is a scale factor. We will chose $f = 2(a+1)$ and $a$ to be a tunable parameter of the filter. The inverse representation is obtained as 
\begin{equation} 
\label{mrp:toquat}
\begin{aligned}
q_s =& \frac{-a\ \norm{\mathbf{p}}^2 + f \sqrt{f^2+(1-a^2) \norm{\mathbf{p}}^2}}{f^2+\norm{\mathbf{p}}^2} \\
\mathbf{\boldsymbol{q}_v} =& f^{-1}(a+q_s) \mathbf{p}
\end{aligned}
\end{equation}


The implemented algorithm for attitude estimation is summarized in the following steps. 

\paragraph{Initialization}
\begin{itemize}
	\item Define the attitude state vector $\boldsymbol{e}_k$. At every iteration, initialize $\boldsymbol{e}_{k-1}^+ = \mathbf{0_3}$.
\end{itemize}

\paragraph{Prediction Step}
\begin{itemize}
	\item Select from $\tilde{\boldsymbol{s}}_{k-1}^{(i)}$  in (\ref{ukf:pred:sigma_points}) the attitude error sigma points $\tilde{\boldsymbol{e}}_{k-1}^{(i)}$, $i = 0 \dots 2 n$. Transform $\tilde{\boldsymbol{e}}_{k-1}^{(i)}$ in delta quaternion sigma points $\delta \tilde{\boldsymbol{q}}_{k-1}^{(i)}$ using MRP (\ref{mrp:toquat}) and multiply it with the estimate of the current attitude quaternion $\hat{\boldsymbol{q}}_{k-1}^+$
	\begin{equation}
	\begin{aligned}
	&\delta \tilde{\boldsymbol{q}}_{k-1}^{(i)} \leftarrow \textbf{MRP}(\tilde{\boldsymbol{e}}_{k-1}^{(i)}) \\
	\tilde{\boldsymbol{q}}_{k-1}^{(i)} = &\delta \tilde{\boldsymbol{q}}_{k-1}^{(i)} \otimes \hat{\boldsymbol{q}}_{k-1}^+ \\
	& i = 0 \dots 2n
	\end{aligned}
	\end{equation}
	
	\item Propagate $\tilde{\boldsymbol{q}}_{k-1}^{(i)}$ through the system dynamic (\ref{ukf:pred:sysdyn}) by storing it in ${\boldsymbol{s}}_{k-1}^-$ to obtain a set of propagated quaternion sigma points $\tilde{\boldsymbol{q}}_{k}^{(i)}$.
	
	\item Average $\tilde{\boldsymbol{q}}_{k}^{(i)}$, $i = 0\dots 2n$ to obtain the predicted attitude quaternion $\hat{\boldsymbol{q}}_{k}^-$. Averaging is computed on the quaternion manifold using the method proposed in \cite{Markley2007}. As an alternative, it is possible to replace the quaternion average with $\tilde{\boldsymbol{q}}_{k}^{(0)}$, as suggested in \cite{Crassidis2003}. This second approach is in general more robust for larger initial errors.
	
	\item Compute the propagated delta quaternions sigma points $\delta \tilde{\boldsymbol{q}}_k^{(i)}$ and obtain a set of delta sigma points $\tilde{\boldsymbol{e}}_k^{(i)}$ by using MRP (\ref{mrp:fromquat}). 
	\begin{equation}
	\begin{aligned}
	&\delta \tilde{\boldsymbol{q}}_k^{(i)} = \hat{\boldsymbol{q}}_{k}^- \otimes (\tilde{\boldsymbol{q}}_k^{(i)})^{-1} \\
	\tilde{\boldsymbol{e}}_k^{(i)} \leftarrow \textbf{MRP}(&\delta \tilde{\boldsymbol{q}}_k^{(i)})\\ &i = 0, \dots 2 n
	\end{aligned}
	\end{equation}
	
	\item Store $\tilde{\boldsymbol{e}}_k^{(i)}$ in $\bar{\tilde{\boldsymbol{s}}}_k^{(i)}$ and compute the predicted error attitude mean $\hat{\boldsymbol{e}}_k^-$ as in \ref{ukf_pred_mean}. Similarly, compute the predicted attitude covariance as in \ref{ukf_pred_cov} using $\hat{\boldsymbol{e}}_k^-$ and $\hat{\boldsymbol{e}}_k^{(i)}$.
	\end{itemize}
	\paragraph{Update Step}
	\begin{itemize}
		\item Given an attitude measurement $\boldsymbol{q}_k^m$, compute the rotation error between $\hat{\boldsymbol{q}}_{k-1}^+$ and $\boldsymbol{q}_k^m$ (\ref{ukf:att:meas}).
		\begin{equation} \label{ukf:att:meas}
		\delta \boldsymbol{q}_k^m = \hat{\boldsymbol{q}}_{k-1}^+ \otimes {(\boldsymbol{q}_k^m)}^{-1}
		\end{equation}
		\item Transform the measured rotation error quaternion $\delta \boldsymbol{q}_k^m$ in the vector  $\boldsymbol{e}_k^m$ using MRP (\ref{mrp:fromquat}). 
		\item Store $\boldsymbol{e}_k^m$ in $\bar{\hat{\boldsymbol{s}}}_k^-$ and compute the updated attitude error mean and covariance as in \ref{ukf_simpl_updt}. 
		\item Retrieve $\hat{\boldsymbol{e}}_k^+$ from $\bar{\hat{\boldsymbol{s}}}_k^+$ and compute the updated error attitude quaternion $\delta \boldsymbol{q}_k^+$ from $\hat{\boldsymbol{e}}_k^+$ using MRP (\ref{mrp:toquat}).
		\item Rotate the predicted attitude quaternion $\hat{\boldsymbol{q}}_k^-$ of $\delta \boldsymbol{q}_k^+$ to obtain the current quaternion estimate of the attitude
		\begin{equation}
		\hat{\boldsymbol{q}}_k^+ = \hat{\boldsymbol{q}}_k^- \otimes \delta \boldsymbol{q}_k^+
		\end{equation}
	\end{itemize}
	
	
	\section{Admittance Controller}
	\label{ch:admc}
	In this chapter we present the controller derived to generate trajectories compliant with the estimated external force and torque, given a reference trajectory or the current pose. In section \ref{sec:admc:forcecontrol} we provide an intuitive explanation of admittance control, while in section \ref{sec:admc:core} we present our admittance controller. In \ref{subsec:admc:robustness} we describe the controller finite state machine introduced to improve the robustness towards noisy and offset-corrupted forces and torque estimates.
	
	\subsection{Intuitive Explanation of Admittance Control}
	\label{sec:admc:forcecontrol}
	Admittance control is based on the idea that the trajectory which guarantees compliance with external force/torque is generated by simulating a \textit{spring-mass-damper} dynamic system. 
	As represented in Figure \ref{pic:admc:intuitive}, the new trajectory is generated as if the MAV, with virtual mass $m_v$, was connected to the desired trajectory via a spring with elastic constant $K$ and via a damper with damping coefficient $c$. The deviation from the desired trajectory is caused by the estimated external force/torque, which excites the virtual mass. 
	
	\begin{figure}[h]
		\centering
		%\includegraphics[width=0.75\textwidth]{images/AdmcConcept.pdf}
		\caption{Intuitive explanation for Admittance Control}
		\label{pic:admc:intuitive}
	\end{figure}
	
	Compliance with external force/torque can be tuned by changing $K$. Increasing values of $K$ simulate a stiffer spring, which in turn yields to better desired trajectory tracking. Conversely, $K = 0$ guarantees full compliance with external forces.
	
	

	
	
	





